Autonomous steady-state quantum magic under local noise

We determine the local reset cost of sustaining quantum magic under continuous depolarization. Static spin interactions convert reset-induced polarization into nonstabilizer correlations. For interactions involving at most $k$ spins and local coherent strength $J$, the optimal strong-noise threshold obeys $K_{\rm on}^{(k)}/\gamma=\Theta_k[(\gamma/J)^{1/(k-1)}]$, where $\gamma$ is the noise rate and $K$ the reset cap. The exponent is uniform in device size, and the two-body leading coefficient is $1/(2\sqrt{2})$. The hierarchy follows from a coherent transition competing with simultaneous local defects. In weak noise, population amplification across growing devices lets the normalized onset cost vanish with static two-body interactions. Entropy balance separately constrains the size and total reset rate required for a fixed global resource. Explicit two-, three-, and four-body dynamics generate magic from free inputs and converge to a unique mixed steady state. A physical two-body construction connects this stationary resource to its coherent budget, control precision, and preparation time.

==> equation_aliases.tex <==
\makeatletter
\AtBeginDocument{%%
\@ifundefined{r@eq:stage3-local-longitudinal-error}{}{%%
\expandafter\let\expandafter\smaliastmp\csname r@eq:stage3-local-longitudinal-error\endcsname
\expandafter\let\csname r@eq:robust-local-field-coordinates\endcsname\smaliastmp}
\@ifundefined{r@s:global:polymer-identity}{}{%%
\expandafter\let\expandafter\smaliastmp\csname r@s:global:polymer-identity\endcsname
\expandafter\let\csname r@s:global:activity-bound\endcsname\smaliastmp}
\@ifundefined{r@s:global:fixed-point-parameters}{}{%%
\expandafter\let\expandafter\smaliastmp\csname r@s:global:fixed-point-parameters\endcsname
\expandafter\let\csname r@s:global:contraction-constants\endcsname\smaliastmp}
\@ifundefined{r@s:global:creator-local}{}{%%
\expandafter\let\expandafter\smaliastmp\csname r@s:global:creator-local\endcsname
\expandafter\let\csname r@s:global:creation-polynomial\endcsname\smaliastmp}
\@ifundefined{r@s:global:creator-local}{}{%%
\expandafter\let\expandafter\smaliastmp\csname r@s:global:creator-local\endcsname
\expandafter\let\csname r@s:global:creator-algebra\endcsname\smaliastmp}
\@ifundefined{r@s:global:weighted-basis}{}{%%
\expandafter\let\expandafter\smaliastmp\csname r@s:global:weighted-basis\endcsname
\expandafter\let\csname r@s:global:decay-denominator\endcsname\smaliastmp}
\@ifundefined{r@s:global:no-jump-generator}{}{%%
\expandafter\let\expandafter\smaliastmp\csname r@s:global:no-jump-generator\endcsname
\expandafter\let\csname r@s:global:dyson\endcsname\smaliastmp}
\@ifundefined{r@s:global:polymer-identity}{}{%%
\expandafter\let\expandafter\smaliastmp\csname r@s:global:polymer-identity\endcsname
\expandafter\let\csname r@s:global:exact-polymer\endcsname\smaliastmp}
\@ifundefined{r@s:global:left-vacancy}{}{%%
\expandafter\let\expandafter\smaliastmp\csname r@s:global:left-vacancy\endcsname
\expandafter\let\csname r@s:global:exact-scale-ratio\endcsname\smaliastmp}
\@ifundefined{r@s:global:final-weights}{}{%%
\expandafter\let\expandafter\smaliastmp\csname r@s:global:final-weights\endcsname
\expandafter\let\csname r@s:global:final-reconstruction\endcsname\smaliastmp}
\@ifundefined{r@s:global:unperturbed-commutator}{}{%%
\expandafter\let\expandafter\smaliastmp\csname r@s:global:unperturbed-commutator\endcsname
\expandafter\let\csname r@s:global:finite-bch\endcsname\smaliastmp}
\@ifundefined{r@s:global:finite-contraction}{}{%%
\expandafter\let\expandafter\smaliastmp\csname r@s:global:finite-contraction\endcsname
\expandafter\let\csname r@s:global:finite-relaxation\endcsname\smaliastmp}
\@ifundefined{r@s:global:multilinear-map}{}{%%
\expandafter\let\expandafter\smaliastmp\csname r@s:global:multilinear-map\endcsname
\expandafter\let\csname r@s:global:fixed-point-map\endcsname\smaliastmp}
\@ifundefined{r@s:global:weighted-basis}{}{%%
\expandafter\let\expandafter\smaliastmp\csname r@s:global:weighted-basis\endcsname
\expandafter\let\csname r@s:global:global-basis\endcsname\smaliastmp}
\@ifundefined{r@s:global:replacement}{}{%%
\expandafter\let\expandafter\smaliastmp\csname r@s:global:replacement\endcsname
\expandafter\let\csname r@s:global:hamiltonian-budget\endcsname\smaliastmp}
\@ifundefined{r@s:global:ball-bound}{}{%%
\expandafter\let\expandafter\smaliastmp\csname r@s:global:ball-bound\endcsname
\expandafter\let\csname r@s:global:lipschitz-bound\endcsname\smaliastmp}
\@ifundefined{r@s:global:replacement}{}{%%
\expandafter\let\expandafter\smaliastmp\csname r@s:global:replacement\endcsname
\expandafter\let\csname r@s:global:model\endcsname\smaliastmp}
\@ifundefined{r@s:global:dissipator}{}{%%
\expandafter\let\expandafter\smaliastmp\csname r@s:global:dissipator\endcsname
\expandafter\let\csname r@s:global:pauli-jumps\endcsname\smaliastmp}
\@ifundefined{r@s:global:parameters}{}{%%
\expandafter\let\expandafter\smaliastmp\csname r@s:global:parameters\endcsname
\expandafter\let\csname r@s:global:pauli-projectors\endcsname\smaliastmp}
\@ifundefined{r@s:global:polymer-activities}{}{%%
\expandafter\let\expandafter\smaliastmp\csname r@s:global:polymer-activities\endcsname
\expandafter\let\csname r@s:global:polymer-polynomial\endcsname\smaliastmp}
\@ifundefined{r@s:global:polymer-smallness}{}{%%
\expandafter\let\expandafter\smaliastmp\csname r@s:global:polymer-smallness\endcsname
\expandafter\let\csname r@s:global:polymer-recursion\endcsname\smaliastmp}
\@ifundefined{r@s:global:finite-minimum}{}{%%
\expandafter\let\expandafter\smaliastmp\csname r@s:global:finite-minimum\endcsname
\expandafter\let\csname r@s:global:positive-contraction-map\endcsname\smaliastmp}
\@ifundefined{r@s:global:reset-decomposition}{}{%%
\expandafter\let\expandafter\smaliastmp\csname r@s:global:reset-decomposition\endcsname
\expandafter\let\csname r@s:global:reference-probabilities\endcsname\smaliastmp}
\@ifundefined{r@s:global:replacement}{}{%%
\expandafter\let\expandafter\smaliastmp\csname r@s:global:replacement\endcsname
\expandafter\let\csname r@s:global:reset-assumptions\endcsname\smaliastmp}
\@ifundefined{r@s:global:dissipator}{}{%%
\expandafter\let\expandafter\smaliastmp\csname r@s:global:dissipator\endcsname
\expandafter\let\csname r@s:global:reset-jumps\endcsname\smaliastmp}
\@ifundefined{r@s:global:local-interaction-sum}{}{%%
\expandafter\let\expandafter\smaliastmp\csname r@s:global:local-interaction-sum\endcsname
\expandafter\let\csname r@s:global:root-denominator\endcsname\smaliastmp}
\@ifundefined{r@s:global:local-interaction-sum}{}{%%
\expandafter\let\expandafter\smaliastmp\csname r@s:global:local-interaction-sum\endcsname
\expandafter\let\csname r@s:global:root-interaction-sum\endcsname\smaliastmp}
\@ifundefined{r@s:global:source-norm}{}{%%
\expandafter\let\expandafter\smaliastmp\csname r@s:global:source-norm\endcsname
\expandafter\let\csname r@s:global:rooted-bound\endcsname\smaliastmp}
\@ifundefined{r@s:global:section-lemma}{}{%%
\expandafter\let\expandafter\smaliastmp\csname r@s:global:section-lemma\endcsname
\expandafter\let\csname r@s:global:section-excitation\endcsname\smaliastmp}
\@ifundefined{r@s:global:section-lemma}{}{%%
\expandafter\let\expandafter\smaliastmp\csname r@s:global:section-lemma\endcsname
\expandafter\let\csname r@s:global:section-identities\endcsname\smaliastmp}
\@ifundefined{r@s:global:weight-submultiplicativity}{}{%%
\expandafter\let\expandafter\smaliastmp\csname r@s:global:weight-submultiplicativity\endcsname
\expandafter\let\csname r@s:global:touching-sum\endcsname\smaliastmp}
\@ifundefined{r@s:global:no-jump-generator}{}{%%
\expandafter\let\expandafter\smaliastmp\csname r@s:global:no-jump-generator\endcsname
\expandafter\let\csname r@s:global:trajectory\endcsname\smaliastmp}
\@ifundefined{r@s:global:reference-state}{}{%%
\expandafter\let\expandafter\smaliastmp\csname r@s:global:reference-state\endcsname
\expandafter\let\csname r@s:global:unperturbed\endcsname\smaliastmp}
\@ifundefined{r@s:global:unperturbed-commutator}{}{%%
\expandafter\let\expandafter\smaliastmp\csname r@s:global:unperturbed-commutator\endcsname
\expandafter\let\csname r@s:global:unperturbed-bch\endcsname\smaliastmp}
}
\makeatother


==> main_citation_numbers.tex <==
\bibcite{Gottesman1997}{{1}{1997}{{Gottesman}}{{}}}
\bibcite{AaronsonGottesman2004}{{2}{2004}{{Aaronson\ and\ Gottesman}}{{}}}
\bibcite{BravyiKitaev2005}{{3}{2005}{{Bravyi\ and\ Kitaev}}{{}}}
\bibcite{Reichardt2005}{{4}{2005}{{Reichardt}}{{}}}
\bibcite{CampbellBrowne2009}{{5}{2009}{{Campbell\ and\ Browne}}{{}}}
\bibcite{CampbellBrowne2010}{{6}{2010}{{Campbell\ and\ Browne}}{{}}}
\bibcite{BravyiHaah2012}{{7}{2012}{{Bravyi\ and\ Haah}}{{}}}
\bibcite{VanDamHoward2009}{{8}{2009}{{van Dam\ and\ Howard}}{{}}}
\bibcite{Veitch2014}{{9}{2014}{{Veitch\ \emph  {et~al.}}}{{Veitch, Mousavian, Gottesman,\ and\ Emerson}}}
\bibcite{ChitambarGour2019}{{10}{2019}{{Chitambar\ and\ Gour}}{{}}}
\bibcite{HowardCampbell2017}{{11}{2017}{{Howard\ and\ Campbell}}{{}}}
\bibcite{SeddonCampbell2019}{{12}{2019}{{Seddon\ and\ Campbell}}{{}}}
\bibcite{WangWildeSu2019}{{13}{2019}{{Wang\ \emph  {et~al.}}}{{Wang, Wilde,\ and\ Su}}}
\bibcite{Pashayan2015}{{14}{2015}{{Pashayan\ \emph  {et~al.}}}{{Pashayan, Wallman,\ and\ Bartlett}}}
\bibcite{BravyiGosset2016}{{15}{2016}{{Bravyi\ and\ Gosset}}{{}}}
\bibcite{Bravyi2019}{{16}{2019}{{Bravyi\ \emph  {et~al.}}}{{Bravyi, Browne, Calpin, Campbell, Gosset,\ and\ Howard}}}
\bibcite{Seddon2021}{{17}{2021}{{Seddon\ \emph  {et~al.}}}{{Seddon, Regula, Pashayan, Ouyang,\ and\ Campbell}}}
\bibcite{HeinrichGross2019}{{18}{2019}{{Heinrich\ and\ Gross}}{{}}}
\bibcite{Warmuz2025}{{19}{2025}{{Warmuz\ \emph  {et~al.}}}{{Warmuz, Dokudowiec, Radhakrishnan,\ and\ Byrnes}}}
\bibcite{LiuWinter2022}{{20}{2022}{{Liu\ and\ Winter}}{{}}}
\bibcite{Leone2022}{{21}{2022}{{Leone\ \emph  {et~al.}}}{{Leone, Oliviero,\ and\ Hamma}}}
\bibcite{Rubboli2024mixedstate}{{22}{2024}{{Rubboli\ \emph  {et~al.}}}{{Rubboli, Takagi,\ and\ Tomamichel}}}
\bibcite{WeiLiu2024}{{23}{2024}{{Wei\ and\ Liu}}{{}}}
\bibcite{Patra2024}{{24}{2024}{{Patra\ \emph  {et~al.}}}{{Patra, Gupta, Ferraro,\ and\ {Sen(De)}}}}
\bibcite{Cao2026}{{25}{2026}{{Cao}}{{}}}
\bibcite{Lyu2026}{{26}{2026}{{Lyu\ \emph  {et~al.}}}{{Lyu, S{\o }rensen,\ and\ Witczak-Krempa}}}
\bibcite{DeOliveira2026Symmetry}{{27}{2026{}}{{de~Oliveira~Junior\ \emph  {et~al.}}}{{de~Oliveira~Junior, Xuereb, Mac{\^e}do, Brask,\ and\ Chaves}}}
\bibcite{Niroula2024}{{28}{2024}{{Niroula\ \emph  {et~al.}}}{{Niroula, White, Wang, Johri, Zhu, Monroe, Noel,\ and\ Gullans}}}
\bibcite{Hou2026}{{29}{2026}{{Hou\ \emph  {et~al.}}}{{Hou, Cao,\ and\ Yang}}}
\bibcite{Zhen2026WeakInjection}{{30}{2026}{{Zhen\ \emph  {et~al.}}}{{Zhen, Yang, Zhu, Chen,\ and\ Wang}}}
\bibcite{Kraus2008}{{31}{2008}{{Kraus\ \emph  {et~al.}}}{{Kraus, B{\"u}chler, Diehl, Kantian, Micheli,\ and\ Zoller}}}
\bibcite{Diehl2008}{{32}{2008}{{Diehl\ \emph  {et~al.}}}{{Diehl, Micheli, Kantian, Kraus, B{\"u}chler,\ and\ Zoller}}}
\bibcite{Verstraete2009}{{33}{2009}{{Verstraete\ \emph  {et~al.}}}{{Verstraete, Wolf,\ and\ Cirac}}}
\bibcite{TicozziViola2012}{{34}{2012}{{Ticozzi\ and\ Viola}}{{}}}
\bibcite{Pastawski2011}{{35}{2011}{{Pastawski\ \emph  {et~al.}}}{{Pastawski, Clemente,\ and\ Cirac}}}
\bibcite{Kapit2016}{{36}{2016}{{Kapit}}{{}}}
\bibcite{Hartmann2006}{{37}{2006}{{Hartmann\ \emph  {et~al.}}}{{Hartmann, D{\"u}r,\ and\ Briegel}}}
\bibcite{Brask2015}{{38}{2015}{{Brask\ \emph  {et~al.}}}{{Brask, Haack, Brunner,\ and\ Huber}}}
\bibcite{HaackJoye2021}{{39}{2021}{{Haack\ and\ Joye}}{{}}}
\bibcite{Mukhopadhyay2018}{{40}{2018}{{Mukhopadhyay}}{{}}}
\bibcite{MartinezAzcona2026}{{41}{2026}{{Martinez-Azcona\ \emph  {et~al.}}}{{Martinez-Azcona, Sarkis, Tkatchenko,\ and\ Chenu}}}
\bibcite{DeOliveira2026Thermal}{{42}{2026{}}{{de~Oliveira~Junior\ \emph  {et~al.}}}{{de~Oliveira~Junior, Mac{\^e}do, Czartowski, Brask,\ and\ Chaves}}}
\bibcite{Xu2026Onset}{{43}{2026}{{Xu}}{{}}}
\bibcite{FuchsVandeGraaf1999}{{44}{1999}{{Fuchs\ and\ van~de Graaf}}{{}}}
\bibcite{GKLS1976}{{45}{1976}{{Gorini\ \emph  {et~al.}}}{{Gorini, Kossakowski,\ and\ Sudarshan}}}
\bibcite{Lindblad1976}{{46}{1976}{{Lindblad}}{{}}}
\bibcite{Evans1977}{{47}{1977}{{Evans}}{{}}}
\bibcite{Spohn1977}{{48}{1977}{{Spohn}}{{}}}
\bibcite{Frigerio1978}{{49}{1978}{{Frigerio}}{{}}}
\bibcite{SupplementalMaterial}{{50}{}{{Sup}}{{}}}
\bibcite{KirkwoodThomas1983}{{51}{1983}{{Kirkwood\ and\ Thomas}}{{}}}
\bibcite{Bravyi2008}{{52}{2008}{{Bravyi\ \emph  {et~al.}}}{{Bravyi, DiVincenzo,\ and\ Loss}}}
\bibcite{Yarotsky2006}{{53}{2006}{{Yarotsky}}{{}}}
\bibcite{DeRoeckSchutz2016}{{54}{2017}{{De~Roeck\ and\ Sch{\"u}tz}}{{}}}
\bibcite{Crawford2015}{{55}{2015}{{Crawford\ \emph  {et~al.}}}{{Crawford, De~Roeck,\ and\ Sch{\"u}tz}}}
\bibcite{KoteckyPreiss1986}{{56}{1986}{{Koteck{\'y}\ and\ Preiss}}{{}}}
\bibcite{BovierZahradnik2000}{{57}{2000}{{Bovier\ and\ Zahradn{\'i}k}}{{}}}
\bibcite{FernandezProcacci2007}{{58}{2007}{{Fern{\'a}ndez\ and\ Procacci}}{{}}}
\bibcite{ScottSokal2005}{{59}{2005}{{Scott\ and\ Sokal}}{{}}}
\bibcite{MannMinko2024}{{60}{2024}{{Mann\ and\ Minko}}{{}}}
\bibcite{BarthelKliesch2012}{{61}{2012}{{Barthel\ and\ Kliesch}}{{}}}
\bibcite{KastoryanoEisert2013}{{62}{2013}{{Kastoryano\ and\ Eisert}}{{}}}
\bibcite{Cubitt2015}{{63}{2015}{{Cubitt\ \emph  {et~al.}}}{{Cubitt, Lucia, Michalakis,\ and\ P{\'e}rez-Garc{\'i}a}}}
\bibcite{Bertini2025}{{64}{2025}{{Bertini\ \emph  {et~al.}}}{{Bertini, De~Sole, Posta,\ and\ Presilla}}}
\bibcite{Temme2010}{{65}{2010}{{Temme\ \emph  {et~al.}}}{{Temme, Kastoryano, Ruskai, Wolf,\ and\ Verstraete}}}
\bibcite{Arad2025}{{66}{2026}{{Arad\ \emph  {et~al.}}}{{Arad, Firanko,\ and\ Gurevich}}}
\bibcite{Kliesch2014}{{67}{2014}{{Kliesch\ \emph  {et~al.}}}{{Kliesch, Gogolin, Kastoryano, Riera,\ and\ Eisert}}}
\bibcite{Bakshi2024}{{68}{2024}{{Bakshi\ \emph  {et~al.}}}{{Bakshi, Liu, Moitra,\ and\ Tang}}}
\bibcite{Putterman2026}{{69}{2026}{{Putterman\ \emph  {et~al.}}}{{Putterman, Zlokapa,\ and\ Cotler}}}
\bibcite{Kiani2026}{{70}{2026}{{Kiani}}{{}}}
\bibcite{TrivediCirac2022}{{71}{2022}{{Trivedi\ and\ Cirac}}{{}}}
\bibcite{GonzalezGarcia2025}{{72}{2025}{{Gonz{\'a}lez-Garc{\'i}a\ \emph  {et~al.}}}{{Gonz{\'a}lez-Garc{\'i}a, Gorshkov, Cirac,\ and\ Trivedi}}}
\bibcite{Sauer2013}{{73}{2013}{{Sauer\ \emph  {et~al.}}}{{Sauer, Gneiting,\ and\ Buchleitner}}}
\bibcite{Reichardt2009}{{74}{2009}{{Reichardt}}{{}}}
\bibcite{Boykin2002}{{75}{2002}{{Boykin\ \emph  {et~al.}}}{{Boykin, Mor, Roychowdhury, Vatan,\ and\ Vrijen}}}
\bibcite{Schulman2005}{{76}{2005}{{Schulman\ \emph  {et~al.}}}{{Schulman, Mor,\ and\ Weinstein}}}
\bibcite{ReebWolf2014}{{77}{2014}{{Reeb\ and\ Wolf}}{{}}}
\bibcite{HaackJoye2024}{{78}{2024}{{Haack\ and\ Joye}}{{}}}
\bibcite{Capel2018}{{79}{2018}{{Capel\ \emph  {et~al.}}}{{Capel, Lucia,\ and\ P{\'e}rez-Garc{\'i}a}}}
\bibcite{Baumgratz2014}{{80}{2014}{{Baumgratz\ \emph  {et~al.}}}{{Baumgratz, Cramer,\ and\ Plenio}}}
\bibcite{Scalici2024Coherence}{{81}{2024}{{Scalici\ \emph  {et~al.}}}{{Scalici, Naseri,\ and\ Streltsov}}}
\bibcite{WignerYanase1963}{{82}{1963}{{Wigner\ and\ Yanase}}{{}}}
\bibcite{Lieb1973}{{83}{1973}{{Lieb}}{{}}}
\bibcite{Yu2017}{{84}{2017}{{Yu}}{{}}}
\bibcite{Takagi2019}{{85}{2019}{{Takagi}}{{}}}
\bibcite{BravyiSW2011}{{86}{2011}{{Bravyi\ \emph  {et~al.}}}{{Bravyi, DiVincenzo,\ and\ Loss}}}
\bibcite{JordanFarhi2008}{{87}{2008}{{Jordan\ and\ Farhi}}{{}}}
\bibcite{OliveiraTerhal2008}{{88}{2008}{{Oliveira\ and\ Terhal}}{{}}}
\bibcite{ReiterSorensen2012}{{89}{2012}{{Reiter\ and\ S{\o }rensen}}{{}}}
\bibcite{Piani2009}{{90}{2009}{{Piani}}{{}}}
\bibcite{Lami2025}{{91}{2025}{{Lami}}{{}}}
\bibcite{Hoeffding1963}{{92}{1963}{{Hoeffding}}{{}}}
\bibcite{Azuma1967}{{93}{1967}{{Azuma}}{{}}}

